Dynamic Treewidth in Logarithmic Time

We present a dynamic data structure that maintains a tree decomposition of width at most $9k+8$ of a dynamic graph with treewidth at most $k$, which is updated by edge insertions and deletions. The amortized update time of our data structure is $2^{O(k)} \log n$, where $n$ is the number of vertices. The data structure also supports maintaining any ``dynamic programming scheme'' on the tree decomposition, providing, for example, a dynamic version of Courcelle's theorem with $O_{k}(\log n)$ amortized update time; the $O_{k}(\cdot)$ notation hides factors that depend on $k$. This improves upon a result of Korhonen, Majewski, Nadara, Pilipczuk, and Soko{\l}owski [FOCS 2023], who gave a similar data structure but with amortized update time $2^{k^{O(1)}} n^{o(1)}$. Furthermore, our data structure is arguably simpler. Our main novel idea is to maintain a tree decomposition that is ``downwards well-linked'', which allows us to implement local rotations and analysis similar to those for splay trees.

==> Preamble.tex <==
\newcommand{\longversion}[1]{{#1}
\newcommand{\shortversion}[1]}
\pdfoutput=1

\usepackage{microtype}
\usepackage{mdframed}
\usepackage{csquotes}
\usepackage[dvipsnames,svgnames,x11names]{xcolor}
\usepackage{soul}
\newcommand{\hlr}[1]{\sethlcolor{Salmon1}\hl{#1}\sethlcolor{yellow}} 
\newcommand{\hlg}[1]{\sethlcolor{PaleGreen2}\hl{#1}\sethlcolor{yellow}}
\newcommand{\hlb}[1]{\sethlcolor{SkyBlue1}\hl{#1}\sethlcolor{yellow}}
\newcommand{\hlo}[1]{\sethlcolor{Apricot}\hl{#1}\sethlcolor{yellow}}
\newcommand{\hly}[1]{\sethlcolor{Gold}\hl{#1}\sethlcolor{yellow}}
\usepackage{listings}
\usepackage{mathrsfs}
\usepackage[mathscr]{euscript}
\usepackage{amsfonts,amsthm,amsmath}
\usepackage{amssymb}
\usepackage{textpos}
\usepackage{amstext}
\usepackage{graphicx,tikz-cd}
\RequirePackage{fancyhdr}
\usepackage{boxedminipage}
\usepackage{algorithm}
\usepackage[noend]{algpseudocode}
\usepackage{graphics}
\usepackage{pgf}
\usepackage{paralist} 
\usepackage{framed}
\usepackage{thm-restate}
\usepackage{thmtools}
\usepackage{enumerate}
\usepackage{float}
\usepackage{xspace}
%\usepackage{todonotes}
%%%%%
\usepackage{graphicx}
\usepackage{caption}
\usepackage{subcaption}
\usepackage{enumitem}
\usepackage{makecell}
\usepackage{thmtools, thm-restate}
\usepackage{thm-autoref}
 \usepackage{mathdots}
%\usepackage{wrapfig}
\usepackage{multirow}
%\usetikzlibrary{cd}
\usepackage{chngcntr}
\usepackage{apptools}
\usepackage{accents}
\AtAppendix{\counterwithin{lemma}{section}}

\usepackage{lineno}
%\linenumbers


\overfullrule=1mm


\usepackage{vmargin}
\setmarginsrb{1in}{1in}{1in}{1in}{0pt}{0pt}{0pt}{6mm}

\newcommand{\myparagraph}[1]{\smallskip\noindent{\textbf{\sffamily #1}}}

\numberwithin{equation}{section}
\newtheorem{theorem}[equation]{Theorem}
\newtheorem{lemma}[equation]{Lemma}
\newtheorem{hypothesis}[equation]{Hypothesis}
\newtheorem{claim}[equation]{Claim}
\newtheorem{definition}[equation]{Definition}
\newtheorem{observation}[equation]{Observation}
\newtheorem{proposition}[equation]{Proposition}
\newtheorem{corollary}[equation]{Corollary}
\newtheorem{mainlemma}[equation]{Main lemma}
%\newtheorem{redrule}[lemma]{Reduction Rule}
%\newtheorem{remark}[lemma]{Remark}
%\newtheorem{reduction}[lemma]{Reduction Rule}
%\newtheorem{conjecture}[lemma]{Conjecture}
\newcommand{\cqed}{\ensuremath{\lhd}}
\makeatletter
\newenvironment{claimproof}{\par
  \pushQED{\cqed}%
  \normalfont \topsep6\p@\@plus6\p@\relax
  \trivlist
  \item\relax
  {\itshape
    Proof of the claim\@addpunct{.}}\hspace\labelsep\ignorespaces
}{%
  \hfill\popQED\endtrivlist\@endpefalse
}
\makeatother


\date{}


\usepackage{booktabs}

\usepackage[pdftex, plainpages = false, pdfpagelabels, 
                 %pdfpagelayout = useoutlines,
                 bookmarks=false,
                 bookmarksopen = true,
                 bookmarksnumbered = true,
                 breaklinks = true,
                 linktocpage,
                 pagebackref,
                 colorlinks = true,  % was true
                 linkcolor = blue,
                 urlcolor  = blue,
                 citecolor = red,
                 anchorcolor = green,
                 hyperindex = true,
                 hypertexnames = false,
                 hyperfigures
                 ]{hyperref}

\usepackage[nameinlink]{cleveref}
\crefname{observation}{Observation}{Observations}
\crefname{claim}{Claim}{Claims}
\crefname{hypothesis}{Hypothesis}{Hypotheses}
\crefname{mainlemma}{Main lemma}{Main lemmas}




\newcommand{\OO}{\mathcal{O}}
\DeclareMathOperator{\polylog}{polylog}


\newcommand{\ttl}{{\sf{``treewidth too large''}}}
\newcommand{\wl}{\mathsf{wl}}
\newcommand{\tw}{\mathsf{tw}}
\newcommand{\autom}{\mathcal{A}}
\newcommand{\run}{\rho}
\newcommand{\seq}{\mathcal{S}}
\newcommand{\pot}{\Phi}
\newcommand{\pott}{\phi}
\newcommand{\su}[1]{\mathcal{H}(#1)}
\newcommand{\width}{\mathsf{width}}
\newcommand{\trace}{\mathsf{trace}}
\newcommand{\anc}{\mathsf{anc}}
\newcommand{\desc}{\mathsf{desc}}
\newcommand{\depth}{\mathsf{depth}}

\newcommand{\cl}{\mathsf{CL}}


\newcommand{\edges}{\ensuremath{\mathsf{edges}}}
\newcommand{\funrestriction}[2]{#1{\restriction_{#2}}}


\newcommand{\chd}{\mathsf{chd}}

\newcommand{\ddeg}{\Delta}

\newcommand{\evaltime}{\tau}
\newcommand{\overheadtime}{\vartheta}

\newcommand{\CMSO}{\mathsf{CMSO}}


%Define in defs
\newcommand{\primal}{\mathcal{P}}
\newcommand{\bd}{\mathsf{bd}}
\newcommand{\bdc}{\lambda}
\newcommand{\co}[1]{\overline{#1}}

\newcommand{\bag}{\textsf{bag}}
\newcommand{\adh}{\mathsf{adh}}
\newcommand{\adhsize}{\mathsf{adhsize}}


\newcommand{\rescliqs}{\triangleleft}
\newcommand{\orescliqs}{\triangleright}


\newcommand{\prud}{\overline{u}}

\newcommand{\vint}{V_{\mathsf{int}}}

\newcommand{\inapp}{$\star$}

\newcommand{\el}{\mathsf{EL}}


\newcommand{\lmap}{\mathcal{L}}
\newcommand{\leaves}{\mathsf{L}}
\newcommand{\Tc}{\mathcal{T}}
\newcommand{\torso}{\mathsf{torso}}

\newcommand{\compset}{\mathfrak{C}}
